Pattern Transfer Learning for Reinforcement Learning in Order Dispatching

Order dispatch is one of the central problems to ride-sharing platforms. Recently, value-based reinforcement learning algorithms have shown promising performance on this problem. However, in real-world applications, the non-stationarity of the demand-supply system poses challenges to re-utilizing data generated in different time periods to learn the value function. In this work, motivated by the fact that the relative relationship between the values of some states is largely stable across various environments, we propose a pattern transfer learning framework for value-based reinforcement learning in the order dispatch problem. Our method efficiently captures the value patterns by incorporating a concordance penalty. The superior performance of the proposed method is supported by experiments.

==> ARCHIVE/packages_old.tex <==
\usepackage[utf8]{inputenc}
\usepackage[left=1.02in, right=1.02in, top=1.1in, bottom=1.05in]{geometry}
\usepackage{array}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{bm}
\usepackage{natbib}
\usepackage{graphicx}
\usepackage{booktabs}
\usepackage{setspace}
\usepackage{textcomp}
\usepackage{enumitem}
\usepackage{datetime2}
\usepackage{multirow}
\usepackage[font=small,labelfont=bf]{caption}
\doublespacing
\DeclareMathOperator*{\argmin}{arg\!min}
\DeclareMathOperator*{\argmax}{arg\!max}

\usepackage{xcolor}



\usepackage{lineno}
\linenumbers




==> Method_Archive.tex <==
% This assumption holds in many applications. 
% For example, in ride-sharing problem, the MDP environment may vary by different days. 
% The value function $V_t$ obtained in day $t$ is calculated under the MDP environment on day $t, t = 1,2, .., T - 1$.
% Another example is the mHealth problem. 
% The patients' body conditions are different, hence the corresponding MDP environment is different.
% However, all patients share some concordance relations such as the glucose increasing after meal.


% We denote the value function as $V_{new}$. 
% [difficult to re-use those datasets]
% [restate the objective - those old datasets]. 
% Challenges: 
% TD learning can not be applied. different environment. 
% \blue{if GIS, not value of one policy, then? how to describe here?}

% Such an estimation can be a subroutine in a policy learning algorithm. 
% For example, in a popular policy learning approach named policy iteration, [some descriptions]

% , denoted as $\widehat{Q}_{new}$
% We follow the policy iteration algorithm in the new environment $\mathcal{M}$. % paradigm
% At each training epoch $k$, we will interact with the environment for multiple 
% with an initial policy $\pi^0$, we follow the policy 
% in MDP environment $\mathcal{M}$ with (near optimal ?) policy $\pi$ 


% Set of pairs. Consider
% We first review a standard method for value estimation. 
% Note that the following Bellman equation holds for any policy $\pi$ in any MDP $\mathcal{M}$:
It is well-known that $Q^\pi$ is the unique solution of the \textit{Bellman equation} $Q = \B^{\pi} Q$, where $\B^{\pi}$ is the \textit{Bellman evaluation operator}, defined as 
\begin{equation*}
\B^{\pi} Q(s,a) = \Mean_{s' \sim \mathcal{P}(\cdot|s,a), a' \sim \pi(\cdot|s')} [r + \gamma Q(s', a')|s,a]. 
    % Q^{\pi}(s,a) = \Mean_{a_{t+1} \sim \pi(s_{t+1}), \mathcal{M}} [r + Q^{\pi}(s_{t+1}, a_{t+1})| s_t = s, a_t = a]
\end{equation*}
The corresponding \textit{Bellman residual operator} is defined as $\R^{\pi} Q = \B^{\pi} Q - Q$. 
Therefore, $Q^\pi$ is the unique solution of $\R^{\pi} Q = 0$. 

Motivated by the above properties, a standard estimator of the value function is the minimize of the
square norm of the empirical Bellman residual: 
\begin{equation*}
    \hat{L}_2(Q) = \frac{1}{n}\sum [\hatR Q(s_i, a_i)]^2
\end{equation*}

\blue{Not consistent. Need either double sampling strategy or Kernelized version}

Policy evaluation itself is of independent interest, and it is also a critical step in many policy optimization algorithms, such as policy iteration or AC. 

%  Bellman equation, given a set of transition generated by policy $\pi$,  so-called \textit{empirical TD erroes}, as follows: 
% \begin{equation*}
%     \widehat{Q}^{\pi} = argmin_Q \Mean_{(s,a, r, s') \sim \mathcal{D}} 
%     [r + V(s') - Q(s, a)]^2
% \end{equation*}

% in didi, deterministic, QV


% set of transitions $\mathcal{D}_{old} = \{(s_i, a_i, r_i, s'_i)\}$ generated by some policies in an MDP environment $\mathcal{M}_{old}$. 
% \hl{If the value function is not for a policy, then what does it mean? how do we say some ASMPs about it?}
% Let the true value function of $\pi$ in environment $\mathcal{M}$ be $Q$, and denote its estimate as $\widehat{Q}$. 
% Let the corresponding bellman operators be $\B^{\pi_{new}}$ and $\R^{\pi_{new}}$. 

% We assume that the value function $V_{old}$ shares the \textbf{concordance relation} with the value function $V_{new}$ in the new MDP environment $\mathcal{M}_{new}$ with policy $\pi_{new}$. 

% estimate $V_{new}$
% Under Assumption \ref{asmp:concordance_V}, we propose to stabilize the value function estimation by minimizing the
% squared empirical Bellman residual with the concordance constraints: 
% \begin{equation*}
% \begin{split}
%     % &\widehat{L}_2(Q) = 
%     % &\widehat{Q}_{new} = arg
%     min_Q \; \frac{1}{n}\sum_i [\widehat{\R}^{\pi_{new}} Q(s_i, a_i)]^2, s.t. \;\;  c(Q, \widehat{Q}; E, \mu) \le \epsilon, \forall j. 
% \end{split}
% \end{equation*}
%     \mathbb{E}_{(s_1, a_1), (s_2, a_2) \sim \mu} \mathbb{I}
% \big\{[Q(s_1, a_1) - Q(s_2, a_2)] [\widehat{Q}(s_1, a_1) < \widehat{Q}(s_2, a_2)] < 0\big\} 

% \mathcal{J}
% \hl{the concordance relationship below can be more concise(<0)}
%  &= \lambda [\sum_{(i,j) \in E: V^{old}_{i,t} < V^{old}_{j,t}}
%  \mathbb{I}(V_{i,t} > V_{j,t}) + \sum_{(i,j) \in E: V^{old}_{i,t} > V^{old}_{j,t}}
%  \mathbb{I}(V_{i,t} < V_{j,t})], 

\begin{equation*}
\begin{split}
    \widehat{Q}_{new} = argmin_Q \; \frac{1}{n}\sum_i [\widehat{\R}^{\pi_{new}} Q(s_i, a_i)]^2
    + \sum \Big\{\lambda * c(Q, \widehat{Q}; E, \mu) \Big\}
\end{split}
\end{equation*}

% We consider $\mathcal{D}$ is composed of two parts, $\mathcal{D}_{old}$ and $\mathcal{D}_{cur}$, and $\mathcal{D}_{cur}$ can be updated with more online collected data. 
% The environment generating $\mathcal{D}_{old}$ can be different with the current environment, and hence the value function learned with $\mathcal{D}_{old}$ can be significantly different with that with $\mathcal{D}_{cur}$. 
% However, we can assume these two value functions share some structural similarities and hence the two data source can be combined in some way. 
% we consider first solving (\ref{formula: TD}) with $\mathcal{D}_{old}$ to obtain $\{V_{i,t}^{old}\}$, and then solving
Specifically, we solve the following problem recursively. For $t = T - 1, T - 2, \dots, 0$: 
\begin{eqnarray}\label{formula:original_optimization}
\begin{split}
    \widehat{V}_{1,t}, \widehat{V}_{2,t}, \dots, \widehat{V}_{N,t} 
    &= \argmin_{\{V_{i,t}\}_{i=1}^N}
     \sum_{j \in \mathcal{D}_{new}(t)} (V_{i,t} - \gamma^{\Delta t(a)} \widehat{V}_{i', t'} - R_{\gamma}(a))^2 \\
     &+ c(\{V_{i,t}\}_{i=1}^N, 
     \{V_{i,t}^{old}\}_{i=1}^N; \lambda), 
\end{split}
\end{eqnarray} 


\begin{equation}\label{formula:objective}
    \begin{split}
    % &= 
    &\sum_{i \le N} \left[\sum_{j \in \mathcal{D}_{new}(i, t)} (V_{i,t} - \gamma^{\Delta t(a)} \widehat{V}_{i', t'} - R_{\gamma}(a))^2\right] \\
     &+ 
     \lambda 
     \end{split}
\end{equation}


% Specifically, we solve the following problem recursively. For $t = T - 1, T - 2, \dots, 0$: 
    % \sum_{(i,j) \in E}\;
    %  \mathbb{I}\{(V_{i,t} > V_{j,t})(V^{old}_{i,t} < V^{old}_{j,t}) < 0
    %  \} \le \epsilon |E|
    %  \sum_{j \in \mathcal{D}( t)} (V_{i,t} - \gamma^{\Delta t(a)} \widehat{V}_{i', t'} - R_{\gamma}(a))^2


% (s1, s2) \in E
where $h(V, V'; E, \mu)$ is the hinge loss, defined as 
\begin{eqnarray}\label{eqn_omega}
\begin{split}
     \mathbb{E}_{s_1, s_2 \sim \mu}
     &\Big\{
          \mathbb{I}
\big[
V(s_1) < V(s_2)
\big] 
\big[ 1 - V'(s_2) + V'(s_1) \big]_+ \\
&+ 
          \mathbb{I}
\big[
V(s_2) < V(s_1)
\big] 
\big[ 1 - V'(s_1) + V'(s_2) \big]_+
     \Big\}
\end{split}
\end{eqnarray} 


==> Optimization.tex <==
For every $i = 1, \dots, N$, we have 
\begin{equation}\label{formula:gradient}
    \begin{split}
   &\frac{\partial}{\partial V_{i,t}}  \mathcal{L}(\{V_{i,t}\}_{i=1}^N;
     \{V_{i,t}^{old}\}_{i=1}^N, \lambda) \\
    &= 
    2 \sum_{j \in \mathcal{D}_{new}(i, t)} (V_{i,t} - \gamma^{\Delta t(a)} \widehat{V}_{i', t'} - R_{\gamma}(a)) \\
     &+ 
    \frac{\partial}{\partial V_{i,t}} \lambda \left[\sum_{(i,j) \in E: V^{old}_{i,t} < V^{old}_{j,t}}
     [1 - (V_{j,t} - V_{i,t})]_{+}
     + \sum_{(i,j) \in E: V^{old}_{i,t} > V^{old}_{j,t}}
     [1 - (V_{i,t} - V_{j,t})]_{+}\right]\\
    &= 
    2 \sum_{j \in \mathcal{D}_{new}(i, t)} (V_{i,t} - \gamma^{\Delta t(a)} \widehat{V}_{i', t'} - R_{\gamma}(a)) \\
     &- 
    \lambda
    \sum_{j: (i,j) \in E}
    \left[ \mathbb{I}(V^{old}_{i,t} < V^{old}_{j,t}, V_{j,t} - V_{i,t} < 1)
     + \mathbb{I}(V^{old}_{i,t} > V^{old}_{j,t}, V_{i,t} - V_{j,t} < 1)
     \right]
     \end{split}
\end{equation}
% \hl{some details about 1 above}


==> Theory.tex <==
\section{Theory}
% 1. better finite-sample estimation performance (n - inf, lam - 0)
% 2. impacts in policy learning?


==> algorithm_1.tex <==
\begin{algorithm}
      \caption{Online-offline Transfer Learning Algorithm.}
  \begin{algorithmic}[1]
  \STATE Initialize random policy $\pi_0$
  \STATE Initialize value function $V^{old}$ and advantage function $A$
  \STATE Initialize replay memory $\mathcal{D}_{old}$ 
 
     \FOR{$t =  1, .., T$}
     	\STATE Generate trajectories $\mathcal{D}_{cur} = \{(s_i, a_i, r_i, s'_i)\}_{i = 1}^{N_t} $ in MDP environment $\mathcal{M}_t$ with policy $\pi_{t - 1}$
     	
     	\STATE (Value Function) Calculate the value function $V_t$ by optimizing the objective function \eqref{formula:objective}.
     	\STATE Update the replay memory $\mathcal{D}_{old} \leftarrow Append(\mathcal{D}_{old}, \mathcal{D}_{cur})$
	    \STATE (Advantage Function) Update the advantage function: 
	    $A_t(s, a) \rightarrow  \alpha (r(s, a) + \gamma V_t(s') - V_t(s)) + (1 - \alpha) A_t(s, a)$ for $(s, a, r, s') \in \mathcal{D}_{old}$
	    \STATE (Policy Update) Obtain the policy $\pi_t$ by greedy method: 
	    $\pi_t(a|s) = 1$ if $a = arg\max A_t(a|s)$
	    \STATE Update the old/historical value function $V^{old} \leftarrow V_t$
	 \ENDFOR 
  
  
  \end{algorithmic}
   \label{algotable: Online-offline}
\end{algorithm}


==> algorithm_2.tex <==
\begin{algorithm}
      \caption{One-Step Transfer Learning Algorithm.}
  \begin{algorithmic}[1]
  % \STATE Initialize random policy $\pi_0$
  %\STATE Initialize value function $V^{old}$
  
  
  \STATE Collect replay memory $\mathcal{D} = \{ \mathcal{D}_1, \mathcal{D}_2, .., \mathcal{D}_{T-1}\}$ from  MDP environment $\mathcal{M}_t$, $t = 1,2,..,T-1$ with behavior policy $\pi_0$
 
     
   \STATE (Value Function) Evaluate the value function $V_T$ by optimizing the objective function \eqref{formula:objective}.
     	
   \STATE (Advantage Function) Obtain the advantage function: 
	    $A_T(s, a) = r(s, a) + \gamma V_T(s') - V_T(s)$ for $(s, a, r, s') \in \mathcal{D}$
   \STATE (Policy Update) Obtain the policy $\pi_T$ by greedy method: 
	    $\pi_T(a|s) = 1$ if $a = arg\max A_T(a|s)$
  \end{algorithmic}
   \label{algotable: One-Step}
\end{algorithm}


==> note.tex <==
\input{Style}
\input{new_commands}



\title{Transfer Learning}
\author{April}
\date{2020/10/24}


\begin{document}

\maketitle

\section{Related work}




borrow general description:

CoRide: Joint Order Dispatching and Fleet Management for Multi-Scale Ride-Hailing Platforms

1. 把每一块cell都当成一个agent？。。
2. 建立HRL，来解决multi-agent setting
3. 把dispatch问题用rank来解决 （fleet control当做fake订单）
4. 用attention来解决multi-scale （这啥）

Main solution： We treat large district as manager agent and small grid as
worker agent, respectively. The manager operates at a lower spatial
and temporal dimension and sets abstract goals which are conveyed
to its workers. The worker takes specific actions and interacts with
environment coordinated with manager-level goal and worker-level
message.

问题：它的item space是啥。。所有订单和车辆的组合 加上 reposition 的可能？每个时刻难道worker的output不一样吗。。




food delivery --> paper review <-- 

1. Integrating Dijkstra’s algorithm into deep inverse reinforcement learning for food delivery route planning
用历史轨迹来找最优的司机路径。background intro可以看看


2. Delivery Scope: A New Way of Restaurant Retrieval For On-demand Food Delivery Service

关注问题：可配送范围。。

topic：
combine online/offline RL framework for 供（supply）需（demand）系统

画图 Figure 1 in accelarating paper

step1: value iteration converge
step2: our penalty is small than 

toy example：

scale 改变， distribution不太变化，customer越来越多。

related work：

zhou fan paper，concur stat related，（RL）， online-offline



\appendix
\newpage

\end{document}

